Software Architecture of Code Analysis Frameworks Matters: The Frama-C Example

Implementing large software, as software analyzers which aim to be used in industrial settings, requires a well-engineered software architecture in order to ease its daily development and its maintenance process during its lifecycle. If the analyzer is not only a single tool, but an open extensible collaborative framework in which external developers may develop plug-ins collaborating with each other, such a well designed architecture even becomes more important. In this experience report, we explain difficulties of developing and maintaining open extensible collaborative analysis frameworks, through the example of Frama-C, a platform dedicated to the analysis of code written in C. We also present the new upcoming software architecture of Frama-C and how it aims to solve some of these issues.

==> eptcsdata.tex <==
\providecommand{\firstpage}{86}
\providecommand{\publicationstatus}{C. Dubois, P. Masci, D. M\'ery (Eds): 2nd International Workshop\\ on Formal Integrated Development Environment (F-IDE 2015) \\
EPTCS 187, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.187.7}{10.4204/EPTCS.187.7}}
\pdfoutput=1

